Beyond Binary: Towards Fine-Grained LLM-Generated Text Detection via Role Recognition and Involvement Measurement

The rapid development of large language models (LLMs), like ChatGPT, has resulted in the widespread presence of LLM-generated content on social media platforms, raising concerns about misinformation, data biases, and privacy violations, which can undermine trust in online discourse. While detecting LLM-generated content is crucial for mitigating these risks, current methods often focus on binary classification, failing to address the complexities of real-world scenarios like human-LLM collaboration. To move beyond binary classification and address these challenges, we propose a new paradigm for detecting LLM-generated content. This approach introduces two novel tasks: LLM Role Recognition (LLM-RR), a multi-class classification task that identifies specific roles of LLM in content generation, and LLM Influence Measurement (LLM-IM), a regression task that quantifies the extent of LLM involvement in content creation. To support these tasks, we propose LLMDetect, a benchmark designed to evaluate detectors' performance on these new tasks. LLMDetect includes the Hybrid News Detection Corpus (HNDC) for training detectors, as well as DetectEval, a comprehensive evaluation suite that considers five distinct cross-context variations and two multi-intensity variations within the same LLM role. This allows for a thorough assessment of detectors' generalization and robustness across diverse contexts. Our empirical validation of 10 baseline detection methods demonstrates that fine-tuned PLM-based models consistently outperform others on both tasks, while advanced LLMs face challenges in accurately detecting their own generated content. Our experimental results and analysis offer insights for developing more effective detection models for LLM-generated content. This research enhances the understanding of LLM-generated content and establishes a foundation for more nuanced detection methodologies.

==> Table/Detection_tasks.tex <==
\begin{table*}[]
\begin{tabular}{llll}
\toprule
Benchmark                  & LLMs Source                                                                                                                                & Language                                                                                                                                                         & Domain                                                                                                                      \\ \midrule
HC3                        & GPT-3.5                                                                                                                                    & English, Chinese                                                                                                                                                 & Question-Answer Pair                                                                                                        \\[0.1cm]
\multirow{3}{*}{MGTBench}  & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}GPT-3.5-turbo, ChatGLM, \\ Dolly, GPT4All, \\ StableLM, Claude\end{tabular}}                    & \multirow{3}{*}{English}                                                                                                                                         & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Scientific Writing, \\ Story Generation,\\ News Writing\end{tabular}}            \\[0.1cm]
                           &                                                                                                                                            &                                                                                                                                                                  &                                                                                                                             \\[0.1cm]
                           &                                                                                                                                            &                                                                                                                                                                  &                                                                                                                             \\[0.1cm]
\multirow{3}{*}{MULTITuDE} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Alpaca-lora, GPT-3.5 Turbo, \\ GPT-4, LLaMA, OPT, \\ OPT-IML-Max, GPT-3.5, Vicuna\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Arabic, Catalan, Chinese, Czech, \\ Dutch, English, German, Portuguese, \\ Russian, Spanish, Ukrainian\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Scientific Writing, \\ News Writing, \\ Social Media\end{tabular}}               \\[0.1cm]
                           &                                                                                                                                            &                                                                                                                                                                  &                                                                                                                             \\[0.1cm]
                           &                                                                                                                                            &                                                                                                                                                                  &                                                                                                                             \\[0.1cm]
GPABech                    & GPT-3.5                                                                                                                                    & English                                                                                                                                                          & Scientific Writing                                                                                                          \\[0.3cm]
\multirow{3}{*}{M4}        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}GPT-4, GPT-3.5, \\ GPT-3, Cohere, \\ Dolly-v2, BLOOMz\end{tabular}}                             & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}English, Chinese, Russian, \\ Urdu, Indonesian, \\ Bulgarian, Arabic\end{tabular}}                                    & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Web Text, Scientific Writing, \\ News Writing, Social Media, \\ QA\end{tabular}} \\
                           &                                                                                                                                            &                                                                                                                                                                  &                                                                                                                             \\
                           &                                                                                                                                            &                                                                                                                                                                  &           \\  \bottomrule                                                                                                               
\end{tabular}
\caption{a}
\label{fig:Detection task}
\end{table*}


==> Table/Feature.tex <==
\begin{figure}[h]
    \centering
    \begin{tabular}{l|rrrrr}
    \hline
    \textbf{Model}      & \textbf{Human} & \textbf{Create} & \textbf{Revise} & \textbf{Extend} & \textbf{Overall} \\ \hline
    \textbf{RoBERTa}    & 47.41          & 68.00           & 41.74           & 51.87           & 52.25            \\
    \textbf{DeBERTa}    & 47.55          & 57.67           & 52.85           & 63.05           & 55.28            \\
    \textbf{Longformer} & 46.67          & 62.47           & 36.94           & 50.12           & 49.05            \\
    \textbf{GPT2-small} & 61.65          & 87.37           & 61.30           & 81.17           & 72.87            \\
    \textbf{GPT2-medium} & 72.79          & 91.92           & 73.97           & 82.71           & 80.35            \\
    \textbf{GPT2-large} & 72.82          & 92.25           & 74.38           & 83.06           & 80.63            \\
    \textbf{Mistral-7b} & 59.00          & 95.29           & 54.40           & 52.79           & 65.37            \\
    \textbf{LLama3-8b}  & 65.09          & 94.33           & 63.01           & 86.51           & 77.24            \\ \hline
    \end{tabular}
    \caption{Performance comparison of different models as Feature Extractors}
    \label{fig:table}
\end{figure}

==> Table/Inherent.tex <==

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \begin{subfigure}[b]{0.45\textwidth}
            \centering
            \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/Ro_TSNE.png} 
            \label{fig:image1}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.45\textwidth}
            \centering
            \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/TSNE_longformer.png} 
            \label{fig:image2}
        \end{subfigure}
        \vfill
        \begin{subfigure}[b]{0.45\textwidth}
            \centering
            \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/De_TSNE.png} 
            \label{fig:image3}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.45\textwidth}
            \centering
            \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/llama_TSNE.png} 
            \label{fig:image4}
        \end{subfigure}
        \caption{t-SNE visualizations of different models}
        \label{fig:tsne_images}
    \end{subfigure}
    % Subfigure (a) for the table
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \begin{tabular}{l|rrrrr}
        \hline
        \textbf{Model}      & \multicolumn{1}{l}{\textbf{Human}} & \multicolumn{1}{l}{\textbf{Create}} & \multicolumn{1}{l}{\textbf{Revise}} & \multicolumn{1}{l}{\textbf{Extend}} & \multicolumn{1}{l}{\textbf{Overall}} \\ \hline
        \textbf{RoBERTa}    & 91.63                     & 89.03                      & 93.51                      & 80.01                      & 88.55                       \\
        \textbf{DeBERTa}    & 86.96                     & 92.59                      & 88.73                      & 79.40                      & 86.92                       \\
        \textbf{Longformer} & 92.12                     & 91.31                      & 90.35                      & 83.57                      & 89.34                       \\
        \textbf{GPT2-small}    & 85.55                     & 88.86                      & 81.18                      & 73.82                      & 82.35                       \\
        \textbf{GPT2-medium} & 87.22          & 90.73           & 84.25           & 78.38           & 85.15            \\
        \textbf{GPT2-large} & 90.32          & 91.21           & 87.19           & 80.65           & 87.34            \\
        \textbf{Mistral-7b} & 94.70          & 89.94           & 94.36           & 85.40           & 91.10            \\
        \textbf{LLama3-8b}  & 95.05                     & 94.45                      & 95.80                      & 92.08                      & 94.35                       \\ \hline
        \end{tabular}
        \caption{Performance comparison of different models}
        \label{fig:table}
    \end{subfigure}
    \hfill
    % Subfigure (b) for the t-SNE images
    \caption{Models' Inherent Distinguishing Capabilities}
    \label{fig:combined}
\end{figure}

==> Table/Poster.tex <==
\begin{table*}[]
\centering
\scalebox{0.95}{
\begin{tabular}{@{}l|rrr|rrr@{}}
\toprule
\multirow{2}{*}{} & \multicolumn{3}{c|}{\textbf{LLM-RR (F1 ↑)}}                & \multicolumn{3}{c}{\textbf{LLM-IM (MSE ↓)}}                \\ \cmidrule(l){2-7} 
                  & \textbf{RoBERTa} & \textbf{DeBERTa} & \textbf{Longformer} & \textbf{RoBERTa} & \textbf{DeBERTa} & \textbf{Longformer} \\ \midrule
\textbf{Base}                           & 99.81            & 99.84            & 99.91               & 0.0027           & 0.0013           & 0.0019              \\ \midrule
\textbf{cross-time}      & 97.20            & 98.76            & 97.05               & 0.0150           & 0.0100           & 0.0077              \\ \midrule
\textbf{cross-prompt} & 95.49            & 95.04            & 96.48               & 0.0126           & 0.0119           & 0.0108              \\ \midrule
\textbf{cross-source}         & 97.59            & 98.66            & 98.75               & 0.0033           & 0.0031           & 0.0035              \\ \midrule
\textbf{cross-cultural}       & 93.96            & 91.11            & 90.67               & 0.0180           & 0.0125           & 0.0134              \\ \midrule
\textbf{cross-domain}         & 65.75            & 78.86            & 71.78               & 0.0375           & 0.0414           & 0.0417              \\ \midrule
\textbf{Overall Average}          & 90.00            & 92.49            & 90.95               & 0.0173           & 0.0158           & 0.0154              \\ \bottomrule
\end{tabular}}
\caption{Generalization performance of PLM-based baseline methods across five cross-context variations.}
\label{tab:Transferability}
\end{table*}

==> Table/TSNE.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/Ro_TSNE.png}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/De_TSNE.png}
    \end{minipage}

    \vspace{0.1cm} 

    \begin{minipage}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/TSNE_longformer.png}
    \end{minipage}
    \begin{minipage}{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/llama_TSNE.png}
    \end{minipage}
\caption{2D t-SNE Plot of Embeddings Computed From Hidden States of Different Pre-Trained Language Models}
\label{fig:TSNE}
\end{figure}

==> Table/data_leakage.tex <==
% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/cm_gpt4_pre_post.png}
%         \caption{Comparison of Confusion Matrices for the LLM-RR Task}
%         \label{fig:confusion_matrix}
%     \end{subfigure}
%     \vspace{0.2cm}  % 调整子图之间的垂直空隙
    
%     \begin{subfigure}{0.5\textwidth}
%         \centering
% \begin{tabular}{@{}l|rrr|rr@{}}
% \toprule
% \multirow{2}{*}{Test Data} & \multicolumn{3}{c|}{LLM-RR (↑)} & \multicolumn{2}{c}{LLM-IM (↓)} \\ \cmidrule(l){2-6} 
%                       & P        & R        & F1       & MSE           & MAE           \\ \midrule
% Pre                   & 49.53    & 48.62    & 40.29    & 0.3079        & 0.4447        \\
% Post                  & 53.52    & 53.64    & 46.06    & 0.2331        & 0.3744        \\ \bottomrule
% \end{tabular}
%         \caption{Performance Comparison on Two Tasks}
%         \label{fig:data leakage}
%     \end{subfigure}
%     \caption{GPT-4o Detector: Comparisons on Pre-release and Post-release Test Data}
%     \label{fig:detection-bias}
% \end{figure}



==> Table/overall_classification.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{@{}c|rrrr|rrr|rrr@{}}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{}} & \multicolumn{4}{c|}{\textbf{Zero-Shot}}                                      & \multicolumn{3}{c|}{\textbf{Feature-based}}                  & \multicolumn{3}{c}{\textbf{PLM-based}}               \\ \cmidrule(l){2-11} 
\multicolumn{1}{l|}{}                  & \textbf{Mistral} & \textbf{Deepseek} & \textbf{llama3-70B} & \textbf{GPT-4o} & \textbf{Entropy} & \textbf{Perplexity} & \textbf{GLTR} & \textbf{Roberta} & \textbf{Longformer} & \textbf{Deberta} \\ \midrule
\textbf{Human}                         & 40.01            & 43.58             & 44.21               & 59.32           & 49.06            & 60.99               & 61.65         & 99.71         & 99.88            & 99.75            \\
\textbf{Create}                        & 0.12             & 21.76             & 49.31               & 64.89           & 66.52            & 77.90                & 87.37         & 99.93         & 99.94            & 99.87            \\
\textbf{Revise}                        & 0.12             & 8.56              & 1.58                & 7.86            & 14.05            & 59.21               & 61.30         & 99.81         & 99.88            & 99.72            \\
\textbf{Extend}                        & 0                & 0.25              & 8.95                & 29.09           & 23.73            & 64.06               & 81.17         & 99.78         & 99.94            & 99.93            \\ \midrule
\textbf{Overall}                       & 10.07            & 18.54             & 26.01               & 40.29           & 38.34            & 65.54               & 72.87         & 99.81         & 99.91            & 99.82            \\ \bottomrule
\end{tabular}
\caption{Performance Results of Different Detector Methods for \textbf{AI-RR Task} on the HNCP Test Set}
\label{tab:classification}
\end{table*}

==> Table/overall_regression.tex <==
\begin{table*}[ht]
\centering
\scalebox{0.92}{
\begin{tabular}{@{}c|r|rrrr|rrr|rrr@{}}
\toprule
\multirow{2}{*}{\textbf{Metric}}  & \multirow{2}{*}{\textbf{Base}} & \multicolumn{4}{c|}{\textbf{Zero-Shot}}                                      & \multicolumn{3}{c|}{\textbf{Feature-based}}                  & \multicolumn{3}{c}{\textbf{PLM-based}}               \\ \cmidrule(l){3-12} 
                                  &                                & \textbf{Mistral} & \textbf{Deepseek} & \textbf{llama3-70B} & \textbf{GPT-4o} & \textbf{Entropy} & \textbf{Perplexity} & \textbf{GLTR} & \textbf{Roberta} & \textbf{Longformer} & \textbf{Deberta} \\ \midrule
\multicolumn{1}{c|}{\textbf{MSE}} & 0.4637                         & 0.4334           & 0.4297            & 0.2488              & 0.3079          & 0.1185           & 0.0663              & 0.0540        & 0.0027        & 0.0019           & 0.0013           \\
\multicolumn{1}{c|}{\textbf{MAE}} & 0.5679                         & 0.5678           & 0.5479            & 0.4353              & 0.4447          & 0.2949           & 0.1984              & 0.1841        & 0.0281        & 0.0222           & 0.0168           \\ \bottomrule
\end{tabular}}
\caption{Performance Results of Different Detector Methods for \textbf{AI-IE Task} on the HNCP Test Set}
\label{tab:regression}
\end{table*}

==> Table/prompt_diversity.tex <==
 \begin{table*}[]
\centering
\begin{tabular}{@{}p{2cm}|p{13cm}@{}}
\toprule
\multicolumn{2}{l}{\textbf{LLM-Creator}} \\ \midrule
\textbf{Prompt1:} & Here is a news article title: \textless{}title\textgreater{} and its description \textless{}description\textgreater{}, write a \textless{}category\textgreater{} news article based on this news article title and description I gave you and return news article as well as your title with the format Title: \_\_ \#\#\# Article: \_\_ (make sure to use \#\#\# as the delimiter). The article should reflect information available up to \textless{}publish date\textgreater{}. \\ \cmidrule(r){1-2}
\textbf{Prompt2:} & Here is a news article title: \textless{}title\textgreater{} and its description \textless{}description\textgreater{}, write a \textless{}category\textgreater{} news article based on this news article title and description I gave you and return news article as well as your title with the format Title: \_\_ \#\#\# Article: \_\_ (make sure to use \#\#\# as the delimiter). \\ \cmidrule(r){1-2}
\textbf{Prompt3:} & Please write a news about \textless{}title\textgreater{}, \textless{}description\textgreater{}. Return news article as well as your title with the format Title: \_\_ \#\#\# Article: \_\_ (make sure to use \#\#\# as the delimiter). \\ \cmidrule(r){1-2}
\textbf{Prompt4:} & Here is a news article title: \textless{}title\textgreater{} and its description \textless{}description\textgreater{}, write a news article in an expert confident voice. Return news article as well as your title with the format Title: \_\_ \#\#\# Article: \_\_ (make sure to use \#\#\# as the delimiter). \\ \cmidrule(r){1-2}
\textbf{Prompt5:} & Please write a news about \textless{}title\textgreater{}, \textless{}description\textgreater{} in a formal scientific writing voice. Return news article as well as your title with the format Title: \_\_ \#\#\# Article: \_\_ (make sure to use \#\#\# as the delimiter). \\ \midrule

\multicolumn{2}{l}{\textbf{LLM-Polisher}} \\ \cmidrule(r){1-2}
\textbf{Prompt1:} & Please polish the following sentences. 

'''\textless{}news article text\textgreater{}''' \\ \cmidrule(r){1-2}
\textbf{Prompt2:} & Please enhance fluency of the following sentences. 

'''\textless{}news article text\textgreater{}''' \\ \cmidrule(r){1-2}
\textbf{Prompt3:} & Please adjust structures of the following sentences.

'''\textless{}news article text\textgreater{}''' \\ \cmidrule(r){1-2}
\textbf{Prompt4:} & Please rewrite the following sentences in a formal scientific writing voice.

'''\textless{}news article text\textgreater{}''' \\ \cmidrule(r){1-2}
\textbf{Prompt5:} & Please polish the following sentences in a humorous voice.

'''\textless{}news article text\textgreater{}''' \\ \midrule

\multicolumn{2}{l}{\textbf{LLM-Extender}} \\ \cmidrule(r){1-2}
\textbf{Prompt1:} & Please complete the following news article. Don't return the given text. 

The news begins with: 

'''\textless{}beginning text\textgreater{}''' 

Continue from here. \\ \cmidrule(r){1-2}
\textbf{Prompt2:} & Please directly continue to write the news (not repeat my provided content): 

'''\textless{}beginning text\textgreater{}''' \\ \cmidrule(r){1-2}
\textbf{Prompt3:} & Please complete the following news article. Don't return the given text.

The text begin with:

'''\textless{}beginning text\textgreater{}''' \\ \cmidrule(r){1-2}
\textbf{Prompt4:} & Complete the following unfinished news article. Don't return the given text.

The news begin with:

'''\textless{}beginning text\textgreater{}''' 

Continue from here. \\ \cmidrule(r){1-2}
\textbf{Prompt5:} & Please directly continue to write the news (not repeat my provided content):

The news begin with:

'''\textless{}beginning text\textgreater{}''' 

Continue from here. \\ \bottomrule
\end{tabular}
\caption{The Diverse Prompts for Cross-prompt of DetectEval}
\label{tab:prompt_diversity}
\end{table*}

==> Table/robustness.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \begin{minipage}{0.48\textwidth}
            \centering
            \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/Extend_length1.png}
            \caption*{Short Text}
            \label{fig:short_text}
        \end{minipage}\hfill
        \begin{minipage}{0.48\textwidth}
            \centering
            \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/Extend_length3.png}
            \caption*{Long Text}
            \label{fig:long_text}
        \end{minipage}
        \caption{Extend Length Experiments}
        \label{fig:combined_texts}
    \end{subfigure}\hfill
    \begin{subfigure}{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/Figure/Polish_times1.png}
        \caption{Polish Times Experiments}
        \label{fig:polish}
    \end{subfigure}
    \caption{Robustness Analysis of AI-IE Task}
    \label{fig:combined_final}
\end{figure}

